Provable Subspace Tracking from Missing Data and Matrix Completion

We study the problem of subspace tracking in the presence of missing data (ST-miss). In recent work, we studied a related problem called robust ST. In this work, we show that a simple modification of our robust ST solution also provably solves ST-miss and robust ST-miss. To our knowledge, our result is the first `complete' guarantee for ST-miss. This means that we can prove that under assumptions on only the algorithm inputs, the output subspace estimates are close to the true data subspaces at all times. Our guarantees hold under mild and easily interpretable assumptions, and allow the underlying subspace to change with time in a piecewise constant fashion. In contrast, all existing guarantees for ST are partial results and assume a fixed unknown subspace. Extensive numerical experiments are shown to back up our theoretical claims. Finally, our solution can be interpreted as a provably correct mini-batch and memory-efficient solution to low-rank Matrix Completion (MC).

==> Tex_Commands.tex <==

%\newcommand{\abs}[1]{\left\vert#1\right\vert}
\newcommand{\set}[1]{\left\{#1\right\}}
\newcommand{\seq}[1]{\left<#1\right>}
\newcommand{\norm}[1]{\left\Vert#1\right\Vert}
\newcommand{\essnorm}[1]{\norm{#1}_{\ess}}
% THEOREM ENVIRON ---------------------------------------------------

%from zcom.tex %\input{zcom}
\newcommand{\bi}{\begin{itemize}} %[<+>]
\newcommand{\ei}{\end{itemize}}
\newcommand{\ben}{\begin{enumerate}}
\newcommand{\een}{\end{enumerate}}
\newcommand{\be}{\protect\[}
\newcommand{\ee}{\protect\]}
\newcommand{\bean}{\begin{eqnarray*} }
\newcommand{\eean}{\end{eqnarray*} }
\newcommand{\bea}{\begin{eqnarray} }
\newcommand{\eea}{\end{eqnarray} }
\newcommand{\ba}{\begin{align*} }
\newcommand{\ea}{\end{align*} }
\newtheorem{remark}[theorem]{Remark}
\newcommand{\nn}{\nonumber}
%\newcommand{\ba}{\begin{array} }
%\newcommand{\ea}{\end{array} }
\newcommand{\re}{\mathbb{R}}
\newcommand{\n}{{\cal N}}



%commands from Dynamic CS and Modified-CS works
\newcommand{\rest}{{T_\text{rest}}}
\newcommand{\zetahat}{\hat{\zeta}}
%\newcommand{\sm}{\text{small}}
\newcommand{\tDelta}{{\tilde{\Delta}}}
\newcommand{\tDeltae}{{\tilde{\Delta}_e}}
\newcommand{\tT}{{\tilde{T}}}
%\newcommand{\add}{{\cal A}}
%\newcommand{\rem}{{\cal R}}
\newtheorem{sigmodel}{Signal Model}

\newcommand{\thr}{{\text{thr}}}
\newcommand{\delthr}{{\text{del-thr}}}
\newcommand{\delbound}{{b}}
\newcommand{\err}{{\text{err}}}
\newcommand{\Q}{{\cal Q}}

\newcommand{\CSres}{{\text{CSres}}}
\newcommand{\diff}{{\text{diff}}}
\newcommand{\Aset}{{\cal A}}
\newcommand{\Rset}{{\cal R}}
\newcommand{\Iset}{{\cal I}}
\newcommand{\Dset}{{\cal D}}
\newcommand{\Sset}{{\cal S}}
\newcommand{\Lset}{{\cal L}}
\newcommand{\Nset}{N}  %{{\cal N}}
\newcommand{\Nhat}{\hat{{\cal N}}}
\newcommand{\N}{{{\cal T}}}
%\newcommand{\del}{\text{del}}
%\newcommand{\Span}{\text{range}}
%\newcommand{\Phat}{\hat{P}}
%\newcommand{\that}{\hat{t}}
%\newcommand{\new}{{\text{new}}}
%\newcommand{\old}{{\text{old}}}
\newcommand{\dif}{{\text{dif}}}
%\newcommand{\thresh}{{\text{thresh}}}
%\newcommand{\Shat}{\hat{S}}
%\newcommand{\lhat}{\hat{\ell}}
\newcommand{\xhat}{\hat{x}}
%\newcommand{\That}{\hat{\mathcal{T}}}
%\newcommand{\T}{\mathcal{T}}
%\newcommand{\SE}{\text{SE}}
\newcommand{\mat}{\mathrm{mat}}
%\newcommand{\train}{{\text{train}}}  %(recursive projected CS)
%\newcommand{\train}{{\text{0}}}  %(recursive projected CS)


\newcommand{\bl}{\begin{frame}}
\newcommand{\el} {\end{frame}}
\newcommand{\hd}{\frametitle}
%\newcommand{\sd}{\frametitle}
\newcommand{\cred}{\color{red}} % \bf
\newcommand{\cb}{\color{blue}}
\newcommand{\cbl}{\color{black}}
\newcommand{\cg}{\color{DarkGreen}}
\newcommand{\im}{\vspace{1mm} \item}
\newcommand{\vs}{\vspace{2mm}}
\newcommand{\vsl}{\vspace{1mm}}
\newcommand{\vsm}{\vspace{-2mm}}
\newcommand{\svdeq}{\overset{\mathrm{SVD}}=}
\newcommand{\evdeq}{\overset{\mathrm{EVD}}=}

\newcommand{\supp}{\text{support}}
\newcommand{\tw}{\tilde{w}}


\renewcommand\thetheorem{\arabic{section}.\arabic{theorem}}

%%% ReProCS Commands %%%%%%%%%%
\newcommand{\wt}{\bm{w}_t}
\newcommand{\mt}{\bm{m}_t}
\newcommand{\xt}{\bm{x}_t}
\newcommand{\x}{\bm{x}}
\newcommand{\xhatt}{\hat{\bm{x}}_t}
\renewcommand{\l}{\bm{\ell}}
\newcommand{\s}{\bm{s}}
\newcommand{\lt}{\bm{\ell}_t}
%\newcommand{\lhat}{\bm{\hat{\ell}}}
\newcommand{\lhat}{\hat{\bm{\ell}}}

\newcommand{\lhatt}{\hat{\l}_t}   %{\bm{y}_t} %{\y_t}
\newcommand{\yt}{\bm{y}_t}
\newcommand{\y}{\bm{y}}
%\newcommand{\wt}{\bm{w}_t}
\newcommand{\w}{\bm{w}}
\renewcommand{\v}{{\bm{v}}}
\newcommand{\vt}{\bm{v}_t}

\renewcommand{\a}{\bm{a}}
\newcommand{\e}{\bm{w}}  %{\bm{e}}
\newcommand{\bnu}{{\bm{\nu}}}
\newcommand{\et}{\bm{w}_t}%{\bm{e}_t}
\newcommand{\Pt}{P_t} %{\bm{P}_t}
\newcommand{\Pj}{\bm{P}_{(j)}}
\newcommand{\Pjm}{\bm{P}_{(j-1)}}
\newcommand{\Pjs}{\bm{P}_{(j),*}}

\newcommand{\ttrain}{t_{\mathrm{train}}}
\newcommand{\rmnew}{\mathrm{new}}
\newcommand{\new}{\mathrm{new}}
\newcommand{\ex}{\mathrm{ex}}

\newcommand{\Pjnew}{\bm{P}_{(j),\mathrm{new}}}
\newcommand{\at}{\bm{a}_t}
\newcommand{\ats}{\bm{a}_{t,*}}
\newcommand{\atnew}{\bm{a}_{t,\mathrm{new}}}
\newcommand{\I}{\bm{I}}
\newcommand{\Lamt}{\bm{\Lambda}_t}
\newcommand{\Lam}{\bm{\Lambda}}
\newcommand{\Lamtnew}{\bm{\Lambda}_{t,\mathrm{new}}}
\newcommand{\Lamtaunew}{\bm{\Lambda}_{\tau,\mathrm{new}}}
\newcommand{\Lamtstar}{\bm{\Lambda}_{t,*}}
\newcommand{\Lamtex}{\bm{\Lambda}_{t}}
%\newcommand{\bm\Sigma}{\bm{\Lambda}_{(j)}}
\newcommand{\T}{\mathcal{T}}
\newcommand{\J}{\mathcal{J}}


\newcommand{\D}{\bm{D}}
\newcommand{\A}{\bm{A}}
\newcommand{\cM}{\hat{\bm{D}}}  % {\mathcal{\bm{M}}}
\newcommand{\cA}{\bm{D}}    %{\mathcal{\bm{A}}}
\newcommand{\cH}{\bm{H}}


\newcommand{\cs}{\text{cs}}
\newcommand{\bigO}{\mathcal{O}}
\newcommand{\bigo}{\mathcal{O}}
\newcommand{\newset}{\mathrm{new-set}}
\newcommand{\old}{\mathrm{old}}
\newcommand{\Shat}{\hat{\bm{s}}}
\newcommand{\shat}{\hat{\bm{s}}}
%\newcommand{\Lhat}{\y}
%\newcommand{\lhat}{\l}

\newcommand{\Ltilde}{\ttilde{\bm{\ell}}}
\newcommand{\Ltil}{\ttilde{\bm{\ell}}}
\renewcommand{\P}{P}  %{\bm{P}}
\newcommand{\U}{\bm{U}}
\newcommand{\V}{\bm{V}}
\newcommand{\R}{\bm{R}}
\newcommand{\ch}{{\mathrm{ch}}}
\newcommand{\fx}{{\mathrm{fix}}}

\newcommand{\mG}{{\mathcal{G}}}
\newcommand{\G}{{\bm{G}}}
\newcommand{\Ghat}{\hat{\bm{G}}}


\renewcommand{\b}{\bm{b}}
\newcommand{\Phat}{\hat{P}}  %{\hat{\bm{P}}}
\newcommand{\Qhat}{\hat{Q}}
\newcommand{\Span}{\operatorname{span}}%{\operatorname{range}}
\newcommand{\del}{\mathrm{del}}
\newcommand{\diag}{\mathrm{diag}}
\newcommand{\add}{\mathrm{add}}%{\mathrm{add}}
\newcommand{\basis}{\operatorname{basis}}
\newcommand{\rank}{\operatorname{rank}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\calc}{\mathcal{C}}
\newcommand{\full}{\mathrm{full}}
\newcommand{\cov}{\operatorname{Cov}}

\newcommand{\train}{\mathrm{train}} %{\mathrm{train}}
\newcommand{\thresh}{\lambda_{\mathrm{thresh}}}  %{\mathrm{thresh}}  %{\hat{\lambda}^-}
\newcommand{\bbbetathresh}{\eta} %{\text{add-thresh}}
\newcommand{\That}{\hat{\mathcal{T}}}
\newcommand{\zetasp}{{\zeta_{*}^+}}
\newcommand{\SE}{\mathrm{SE}}
\newcommand{\egam}{\Gamma^e}
\newcommand{\Ijk}{\mathcal{I}_{k}}
\newcommand{\that}{{\hat{t}}}
\newcommand{\rmend}{\mathrm{end}}
\newcommand{\M}{\bm{M}}
\newcommand{\range}{\operatorname{span}}%{\operatorname{range}}
\newcommand{\llceil}{\left\lceil}
\newcommand{\rrceil}{\right\rceil}
\newcommand{\llfloor}{\left\lfloor}
\newcommand{\rrfloor}{\right\rfloor}
\newcommand{\uhat}{{\hat{u}}}
%\newcommand{\lammin}{{\hat{\lambda}_{\train}^-}}
\newcommand{\lammin}{{\lambda}^-}
\newcommand{\lamtrain}{{\lambda}^-} %{{\hat{\lambda}_{\train}^-}}
\newcommand{\jhat}{j}%{\hat{\jmath}}

\newcommand{\rrho}{\rho}
%\newcommand{\Ijk}{\mathcal{I}_{k}}
\newcommand{\Ijkt}{\ttilde{\mathcal{I}}_{k}}
\newcommand{\ghatp}{\hat{g}}%{\hat{g}^+}
\newcommand{\calGjk}{\mathcal{G}_{k}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\Lamcl}{\bm{\Lambda}_{(j),\mathrm{cl}}}
\newcommand{\bnut}{{\bnu}_t}
\newcommand{\bmG}{\bm{G}}
\renewcommand{\L}{\bm{L}}
\renewcommand{\S}{\bm{S}}
\newcommand{\Y}{\bm{Y}}
\newcommand{\W}{\bm{W}}
\newcommand{\bE}{\bm{E}}
\newcommand{\F}{\bm{F}}
\newcommand{\bF}{\bm{F}}
\newcommand{\bR}{\bm{R}}

\renewcommand{\H}{\bm{H}}


\newcommand{\outfrac}{\text{outlier-fraction}}
\newcommand{\outfracrow}{\text{outlier-fraction-row}}
\newcommand{\outfraccol}{\text{outlier-fraction-col}}

\newcommand{\tmax}{d}

\newcommand{\matr}[2]{ \left[\begin{array}{cc}
     #1 \\
     #2
   \end{array}
  \right]
  }

\renewcommand{\implies}{\Rightarrow}


==> extensions.tex <==
\subsection{Extensions of the basic NORST-miss approach} \label{sec:ext}
%\color{blue}
%??pn-need lot of edits here to the time/memory complexity. Also, good idea to include a theoretical table here that compares some  of the recent algorithms and all the NORST variants here.
%\color{black}

%In this section we describe two simple heuristics that help improve the performance of the basic NORST-miss idea described earlier. The same ideas in fact can also be used to improve the practical performance of NORST-miss-robust and in fact also of the original NORST algorithm for RST \cite{rrpcp_icml}.

%{\cb In this section, we provide three extensions of the basic Algorithm \ref{algo:NORST-st-basic}. The first extension borrows the idea of GROUSE/PETRELS and 

In this section we describe three simple heuristics that help improve the performance of the basic NORST-miss idea described earlier. The first heuristic allows us to tolerate much higher fraction of outliers once a good enough estimate of the subspace is obtained. The second and third heuristics help to practically improve the performance of Algorithm \ref{algo:NORST-st-basic}. The same ideas in fact can also be used to improve the performance of Algorithm \ref{algo:auto-dyn-rmc} and in fact also of the original NORST algorithm for RST \cite{rrpcp_icml}.


{\cb
\subsubsection{Sample-Efficient-NORST-miss} We explain here a simple modification of NORST-miss that will reduce its sample complexity under the i.i.d. Bernoulli model. The reason that NORST-miss needs many more observed entries is because of the projected LS step which solves for the missing entries vector, $\z_t$, after projecting $\yt$ orthogonal to $\Phat_{(t-1)}$. This step is computing the pseudo-inverse of $(\I - \Phat_{(t-1)} \Phat_{(t-1)}{}')_{\Tmisst}$. Our bound on $\missfraccol$ helps ensure that this matrix is well conditioned for any set $\Tmisst$ of size at most $\missfraccol \cdot n$.
Notice however that we prove that NORST-miss recovers $\P_j$ to $\epsilon$ accuracy with a delay of just $(K+2) \alpha = C r \log n \log(1/\epsilon)$. Once the subspace has been recovered to $\zz$ accuracy, there is no need to use projected LS to recover $\z_t$. One just needs to recover $\at$ given a nearly perfect subspace estimate and the observed entries. This can be done more easily as follows (borrows PETRELS idea): let $\Phat_{(t)} \leftarrow \Phat_{(t-1)}$, solve for $\at$ as $\hat\a_t:= (\I_{\Omega_t}{}' \Phat_{(t)})^{\dagger} \I_{\Omega_t}{}'\y_t$, and set $\lhat_t \leftarrow \Phat_{(t)} \hat\a_t$. Recall here that $\Omega_t = \Tmisst^c$. If the set of observed or missing entries was i.i.d. Bernoulli for just the later time instants, this approach will only need $\Omega (r \log r \log^2 n)$ samples at each time $t$, whp. This follows from  \cite[Lemma 3]{laura_subspace_match}.
Thus, with this approach, if $d \le n$, the number of observed entries needed is only
$n(1-1/r) K \alpha + C r \log r \log^2 n (d - K \alpha) = C[ n(1-1/r) r \log n \log(1/\epsilon) + d r \log r \log^2 n ] = \Omega ( n r \log^3 n \log(1/\epsilon) )$ as long as the observed entries follow the i.i.d. Bernoulli model for the time instants after the first $K \alpha$ time instants after a subspace change. Or, we need the observed entries to be i.i.d. Bernoulli($1 - c/r)$) for first $K \alpha$ frames and i.i.d. Bernoulli($ r\log r (\log n)^2 / n$) afterwards.
}
\subsubsection{NORST-sliding-window} In the basic NORST approach we use a different set of estimates $\lhat_t$ for each subspace update step. So, for example, the first subspace estimate is computed at $\that_j + \alpha-1$ using $[\lhat_{\that_j}, \lhat_{\that_j+1}, \dots, \lhat_{\that_j+\alpha-1}]$; the second is computed at $\that_j+2 \alpha-1$ using $[\lhat_{\that_j+\alpha}, \lhat_{\that_j+ \alpha+1}, \dots, \lhat_{\that_j+2\alpha-1}]$; and so on. This is done primarily to ensure mutual independence of the set of $\lt$'s in each interval because this is what makes the proof easier (allows use of matrix Bernstein for example). However, in practice, we can get faster convergence to an $\epsilon$-accurate estimate of $\P_j$, by removing this restriction. This approach is of course motivated by the sliding window idea that is ubiquitous in signal processing. For any sliding-window method, there is the window length which we keep as $\alpha$ and the hop-length which we denote by $\beta$.

Thus, NORST-sliding-window ($\beta$) is Algorithm \ref{algo:NORST-st-basic} with the following change: compute $\Phat_{j,1}$ using $[\lhat_{\that_j}, \lhat_{\that_j+ \alpha+1}, \dots, \lhat_{\that_j+\alpha-1}]$; compute $\Phat_{j,2}$ using $[\lhat_{\that_j + \beta}, \lhat_{\that_j+ \beta+1}, \dots, \lhat_{\that_j+\beta  + \alpha-1}]$; compute $\Phat_{j,3}$ using $[\lhat_{\that_j +2 \beta}, \lhat_{\that_j+ 2\beta+1}, \dots, \lhat_{\that_j+2\beta  + \alpha-1}]$;  and so on.
 Clearly $\beta < \alpha$ and $\beta=\alpha$ returns the basic NORST-miss.


%The memory complexity increases slightly (only in constant factors) and the storage required for this case is $\mathcal{O}(n(\alpha+\beta)) = \mathcal{O}(n \alpha)$ since $\beta > \alpha$ is not a practically valid setting. Finally, notice that when $\alpha=\beta$, we recover the NORST-basic algorithm. Furthermore, we see that the number of subspace update steps here is $\mathcal{O}\left((\tmax-\alpha)/\beta \right)$ and thus this increases the complexity to $\mathcal{O}\left(n \tmax \alpha r \log(1/\epsilon) /\beta  \right)$ which is bigger by a factor of $\mathcal{O}(\alpha/\beta)$.

\subsubsection{NORST-buffer} Another question if we worry only about practical performance is whether re-using the same $\alpha$ data samples $\yt$ in the following way helps: {\cb At $t = \that_j + k\alpha -1$, the $k$-th estimate is improved $R$ times as follows. First we obtain $\Lhat_{t;\alpha}:=[\lhat_{t-\alpha+1}, \lhat_{t-\alpha+2}, \dots \lhat_t]$ which are used to compute $\Phat_{j,k}$ via $r$-SVD. Let us denote this by $\Phat_{j,k}^{0}$. Now, we use this estimate to obtain a second, and slightly more refined estimate of the same $\L_{t;\alpha}$. We denote these as $\Lhat_{t;\alpha}^{(1)}$ and use this estimate to get $\Phat_{j,k}^{(1)}$.} This process is repeated for a total of $R + 1$ (reuse) times. We noticed that using $R=4$ suffices in most synthetic data experiments and for real data, $R=0$ (which reduces to the basic NORST algorithm) suffices.
This variant has the same memory requirement as NORST-original. The time complexity, however, increases by a factor of $R + 1$ since there are $R + 1$ times more subspace estimation steps. In other words, the computational complexity increases to $\mathcal{O}(n d r (R + 1) \log(1/ \epsilon))$.

%We can update our estimation of the subspace after each $\alpha$-frames and then go back and reuse the final estimation-that we had after $\alpha$ frames-to the same frame of samples so that we'll have more accurate estimation of the subspace. Then, we input it as the initial value to the next batch of samples.\\


%\subsubsection{Hybrid: Buffer + Sliding Window}
%We can combine the two previous ideas and come up with hybrid variants that exploit the advantages of both extensions. We provide detailed experimental validation of the different extensions in Sec \ref{sec:sims_main}. 


